Enhancing Automated Software Traceability by Transfer Learning from Open-World Data

Software requirements traceability is a critical component of the software engineering process, enabling activities such as requirements validation, compliance verification, and safety assurance. However, the cost and effort of manually creating a complete set of trace links across natural language artifacts such as requirements, design, and test-cases can be prohibitively expensive. Researchers have therefore proposed automated link-generation solutions primarily based on information-retrieval (IR) techniques; however, these solutions have failed to deliver the accuracy needed for full adoption in industrial projects. Improvements can be achieved using deep-learning traceability models; however, their efficacy is impeded by the limited size and availability of project-level artifacts and links to serve as training data. In this paper, we address this problem by proposing and evaluating several deep-learning approaches for text-to-text traceability. Our method, named NLTrace, explores three transfer learning strategies that use datasets mined from open world platforms. Through pretraining Language Models (LMs) and leveraging adjacent tracing tasks, we demonstrate that NLTrace can significantly improve the performance of LM based trace models when training links are available. In such scenarios NLTrace outperforms the best performing classical IR method with an 188% improvement in F2 score and 94.01% in Mean Average Precision (MAP). It also outperforms the general LM based trace model by 7% and 23% for F2 and MAP respectively. In addition, NLTrace can adapt to low-resource tracing scenarios where other LM models can not. The knowledge learned from adjacent tasks enables NLTrace to outperform VSM models by 28% F2 on generation challenges when presented with a small number of training examples.

==> Questions.tex <==
1. Why do you believe that Single BERT architecture is the right one. Just because it worked for NL-PL, does that mean it should also be best for NL to NL.

TODO check list:
- Fig.~ to Figure
- Grammar check 

==> tables/combine_transfer.tex <==
\begin{table*}[t!]
	\centering
	\caption{Combine three transfer learning strategies for completion and extension problem }
	    \begin{subtable}[h]{\textwidth}
	    \centering
        \begin{tabular}{c|cc|cc|cc|cc|cc}
        \toprule \hline
        Completion & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{PTC } & \multicolumn{2}{c|}{Drone} & \multicolumn{2}{c}{CM1} & \multicolumn{2}{c}{Avg Improve} \\
        & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP \\ \hline
        Bert & 0.599 & 0.610 & 0.404 & 0.703 & 0.677 & 0.864 & 0.503 & 0.628 & - & - \\
        SciBert & 0.602 & 0.664 & 0.441 & 0.740 & 0.683 & 0.904 & 0.578 & 0.705 & 6.33\% & 7.74\% \\
        G-CLS & 0.610 & 0.679 & 0.439 & 0.733 & 0.718 & 0.948 & 0.626 & 0.817 & 10.21\% & 13.84\% \\
        P-CLS & 0.616 & 0.641 & 0.412 & 0.692 & 0.715 & 0.918 & 0.592 & 0.772 & 6.96\% & 8.18\% \\
        GP-CLS & 0.591 & 0.625 & 0.371 & 0.727 & 0.683 & 0.904 & 0.556 & 0.686 & 0.47\% & 4.95\% \\
        SE-G-CLS & 0.616 & 0.641 & 0.412 & 0.692 & 0.715 & 0.918 & 0.592 & 0.772 & 6.96\% & 8.18\% \\
        P-Scibert & 0.604 & 0.623 & 0.433 & 0.720 & 0.717 & 0.924 & 0.433 & 0.756 & 0.02\% & 8.00\% \\
        SE-SciBert & 0.614 & 0.634 & 0.384 & 0.610 & 0.688 & 0.901 & 0.319 & 0.479 & -9.39\% & -7.16\% \\
        \end{tabular}

        \label{tab:ctx_acc}
        \end{subtable}
        
        \begin{subtable}[h]{\textwidth}
            \centering
            \begin{tabular}{c|cc|cc|cc|cc|cc}
             \toprule \hline
            Expansion & \multicolumn{2}{c|}{CCHIT} & \multicolumn{2}{c|}{PTC } & \multicolumn{2}{c|}{Drone} & \multicolumn{2}{c}{CM1} & \multicolumn{2}{c}{Avg Improve} \\
            & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP & F2 & MAP \\ \hline
            Bert & 0.284 & 0.211 & 0.488 & 0.580 & 0.541 & 0.716 & 0.318 & 0.258 & - & - \\
            SciBert & 0.384 & 0.295 & 0.493 & 0.634 & 0.589 & 0.713 & 0.512 & 0.409 & 26.65\% & 26.81\% \\
            G-CLS & 0.392 & 0.317 & 0.476 & 0.588 & 0.611 & 0.743 & 0.515 & 0.423 & 27.69\% & 29.87\% \\
            P-CLS & 0.371 & 0.253 & 0.479 & 0.580 & 0.608 & 0.747 & 0.479 & 0.394 & 23.01\% & 19.32\% \\
            GP-CLS & 0.376 & 0.274 & 0.444 & 0.565 & 0.552 & 0.690 & 0.422 & 0.395 & 14.60\% & 19.22\% \\
            SE-G-CLS & & & & & & & & & & \\
            P-Scibert & 0.337 & 0.314 & 0.469 & 0.599 & 0.671 & 0.760 & 0.461 & 0.413 & 21.06\% & 29.64\% \\ 
            SE-SciBert & \nmark{0.399} & \nmark{0.303} & 0.470 & 0.582 & 0.597 & 0.770 & 0.350 & 0.314 & 14.32\% & 18.31\% \\\hline
            \end{tabular}

            \label{tab:ctx_acc}
        \end{subtable}
\end{table*}
